Librarian Agents: Training LLMs to Curate Long-Context Workspaces that Anticipate Future Queries

Reasoning over long document contexts remains a challenge for large language models (LLMs). Standard retrieval methods are inherently reactive, bottlenecking agents with complex, cross-document reasoning at inference time, while precomputed structures like knowledge graphs often fall short because they rely on rigid heuristics. Instead, can we allow agents to perform anticipatory directed curation: learning to proactively reorganize unstructured corpora prior to inference to efficiently serve diverse future queries. We build on a key asymmetry in modern agentic harnesses (e.g., Claude Code): while LLM agents are adept at navigating existing filesystems to solve an immediate task, they are rarely trained to construct reusable workspaces for future use. To instantiate this capability, we introduce Librarian Agents, a framework in which a builder agent transforms raw documents into a hierarchical filesystem of synthetic files and reference links, which forms a workspace tailored for a downstream answering agent. We formulate workspace construction as a Markov decision process and optimize the builder policy via reinforcement learning to directly maximize downstream answering accuracy. Empirically, Librarian Agents outperforms the strongest retrieval and precomputation baselines by 33 percentage points on BrowseComp-Plus, amortizes upfront construction costs across repeated queries, and generalizes zero-shot to unseen domains on BRIGHT with a 31-point average accuracy improvement.

==> sections/statements.tex <==
\section{Reproducibility Statement}
We describe the memory-construction algorithm and GRPO objective in Section~\ref{sec:methods} and Algorithm~\ref{alg:memory-construction}. Appendix~\ref{app:hyperparam} reports the builder model, optimization settings, reward and probe schedule, generation budgets, and evaluation decoding parameters. Appendix~\ref{app:tool-use} specifies the filesystem action space, while Appendix~\ref{app:prompts} provides the builder, answering-agent, judge, and baseline prompts. We will release the code, training scripts, and evaluation framework under the MIT License, and the synthesized filesystem artifacts, logs, and evaluation results under CC BY 4.0, subject to the underlying datasets' licensing terms.

